Towards coercive boundary element methods for the wave equation

In this note, we discuss the ellipticity of the single layer boundary integral operator for the wave equation in one space dimension. This result not only generalizes the well-known ellipticity of the energetic boundary integral formulation in $L^2$, but it also turns out to be a particular case of a recent result on the inf-sup stability of boundary integral operators for the wave equation. Instead of the time derivative in the energetic formulation, we use a modified Hilbert transformation, which allows us to stay in Sobolev spaces of the same order. This results in the applicability of standard boundary element error estimates, which are confirmed by numerical results.

==> Eigenwerte.tex <==
   1.000000000000000   0.000000000000000
   1.200000000000000   1.000000000001231
   1.400000000000000   1.000000000002423
   1.600000000000000   1.000000000003623
   1.800000000000000   1.000000000003647
   2.000000000000000   1.000000000002054
   2.200000000000000   1.414213562373790
   2.400000000000000   1.414213562374519
   2.600000000000000   1.414213562374119
   2.800000000000000   1.414213562375205
   3.000000000000000   1.414213562374685
   3.200000000000000   1.618033988750429
   3.400000000000000   1.618033988750859
   3.600000000000000   1.618033988751063
   3.800000000000000   1.618033988751212
   4.000000000000000   1.618033988750424
   4.200000000000000   1.732050807569146
   4.400000000000000   1.732050807569347
   4.600000000000000   1.732050807569571
   4.800000000000001   1.732050807569474
   5.000000000000000   1.732050807569375
   5.200000000000000   1.801937735805083
   5.400000000000000   1.801937735805304
   5.600000000000001   1.801937735805474
   5.800000000000001   1.801937735805445
   6.000000000000000   1.801937735805289
   6.200000000000000   1.847759065022826
   6.400000000000000   1.847759065022973
   6.600000000000001   1.847759065022782
   6.800000000000001   1.847759065022993
   7.000000000000000   1.847759065022944
   7.200000000000000   1.879385241571966
   7.400000000000000   1.879385241572016
   7.600000000000001   1.879385241572113
   7.800000000000001   1.879385241572081
   8.000000000000000   1.879385241571949
   8.199999999999999   1.902113032590428
   8.400000000000000   1.902113032590473
   8.600000000000001   1.902113032590510
   8.800000000000001   1.902113032590530
   9.000000000000000   1.902113032590557
   9.200000000000001   1.918985947229077
   9.400000000000000   1.918985947229105
   9.600000000000000   1.918985947229111
   9.800000000000001   1.918985947229245
  10.000000000000000   1.918985947229135
  10.200000000000001   1.931851652578267
  10.400000000000000   1.931851652578229
  10.600000000000000   1.931851652578327
  10.799999999999999   1.931851652578328
  11.000000000000000   1.931851652578340
  11.199999999999999   1.941883634852201
  11.400000000000000   1.941883634852235
  11.600000000000000   1.941883634852235
  11.799999999999999   1.941883634852252
  12.000000000000000   1.941883634852226
  12.199999999999999   1.949855824363762
  12.399999999999999   1.949855824363732
  12.600000000000000   1.949855824363787
  12.800000000000001   1.949855824363810
  13.000000000000000   1.949855824363772
  13.199999999999999   1.956295201467666
  13.399999999999999   1.956295201467705
  13.600000000000000   1.956295201467663
  13.800000000000001   1.956295201467749
  14.000000000000000   1.956295201467705
  14.199999999999999   1.961570560806515
  14.399999999999999   1.961570560806519
  14.600000000000000   1.961570560806559
  14.800000000000001   1.961570560806556
  15.000000000000000   1.961570560806570
  15.199999999999999   1.965946199367861
  15.399999999999999   1.965946199367864
  15.600000000000000   1.965946199367868
  15.800000000000001   1.965946199367860
  16.000000000000000   1.965946199367851
  16.199999999999999   1.969615506024469
  16.399999999999999   1.969615506024466
  16.600000000000001   1.969615506024478
  16.800000000000001   1.969615506024490
  17.000000000000000   1.969615506024461
  17.199999999999999   1.972722606805498
  17.399999999999999   1.972722606805484
  17.600000000000001   1.972722606805503
  17.800000000000001   1.972722606805521
  18.000000000000000   1.972722606805518
  18.199999999999999   1.975376681190322
  18.399999999999999   1.975376681190326
  18.600000000000001   1.975376681190311
  18.800000000000001   1.975376681190320
  19.000000000000000   1.975376681190334
  19.199999999999999   1.977661652450297
  19.399999999999999   1.977661652450292
  19.600000000000001   1.977661652450319
  19.800000000000001   1.977661652450319
  20.000000000000000   1.977661652450300


==> KonstanteAimi.tex <==
   1.000000000000000   0.000000000000000
   1.200000000000000   1.000000000000000
   1.400000000000000   1.000000000000000
   1.600000000000000   1.000000000000000
   1.800000000000000   1.000000000000000
   2.000000000000000   1.000000000000000
   2.200000000000000   1.414213562373095
   2.400000000000000   1.414213562373095
   2.600000000000000   1.414213562373095
   2.800000000000000   1.414213562373095
   3.000000000000000   1.414213562373095
   3.200000000000000   1.618033988749895
   3.400000000000000   1.618033988749895
   3.600000000000000   1.618033988749895
   3.800000000000000   1.618033988749895
   4.000000000000000   1.618033988749895
   4.200000000000000   1.732050807568877
   4.400000000000000   1.732050807568877
   4.600000000000000   1.732050807568877
   4.800000000000001   1.732050807568877
   5.000000000000000   1.732050807568877
   5.200000000000000   1.801937735804838
   5.400000000000000   1.801937735804838
   5.600000000000001   1.801937735804838
   5.800000000000001   1.801937735804838
   6.000000000000000   1.801937735804838
   6.200000000000000   1.847759065022573
   6.400000000000000   1.847759065022573
   6.600000000000001   1.847759065022573
   6.800000000000001   1.847759065022573
   7.000000000000000   1.847759065022573
   7.200000000000000   1.879385241571817
   7.400000000000000   1.879385241571817
   7.600000000000001   1.879385241571817
   7.800000000000001   1.879385241571817
   8.000000000000000   1.879385241571817
   8.199999999999999   1.902113032590307
   8.400000000000000   1.902113032590307
   8.600000000000001   1.902113032590307
   8.800000000000001   1.902113032590307
   9.000000000000000   1.902113032590307
   9.200000000000001   1.918985947228995
   9.400000000000000   1.918985947228995
   9.600000000000000   1.918985947228995
   9.800000000000001   1.918985947228995
  10.000000000000000   1.918985947228995
  10.200000000000001   1.931851652578137
  10.400000000000000   1.931851652578137
  10.600000000000000   1.931851652578137
  10.799999999999999   1.931851652578137
  11.000000000000000   1.931851652578137
  11.199999999999999   1.941883634852104
  11.400000000000000   1.941883634852104
  11.600000000000000   1.941883634852104
  11.799999999999999   1.941883634852104
  12.000000000000000   1.941883634852104
  12.199999999999999   1.949855824363647
  12.399999999999999   1.949855824363647
  12.600000000000000   1.949855824363647
  12.800000000000001   1.949855824363647
  13.000000000000000   1.949855824363647
  13.199999999999999   1.956295201467611
  13.399999999999999   1.956295201467611
  13.600000000000000   1.956295201467611
  13.800000000000001   1.956295201467611
  14.000000000000000   1.956295201467611
  14.199999999999999   1.961570560806461
  14.399999999999999   1.961570560806461
  14.600000000000000   1.961570560806461
  14.800000000000001   1.961570560806461
  15.000000000000000   1.961570560806461
  15.199999999999999   1.965946199367804
  15.399999999999999   1.965946199367804
  15.600000000000000   1.965946199367804
  15.800000000000001   1.965946199367804
  16.000000000000000   1.965946199367804
  16.199999999999999   1.969615506024416
  16.399999999999999   1.969615506024416
  16.600000000000001   1.969615506024416
  16.800000000000001   1.969615506024416
  17.000000000000000   1.969615506024416
  17.199999999999999   1.972722606805445
  17.399999999999999   1.972722606805445
  17.600000000000001   1.972722606805445
  17.800000000000001   1.972722606805445
  18.000000000000000   1.972722606805445
  18.199999999999999   1.975376681190276
  18.399999999999999   1.975376681190276
  18.600000000000001   1.975376681190276
  18.800000000000001   1.975376681190276
  19.000000000000000   1.975376681190276
  19.199999999999999   1.977661652450257
  19.399999999999999   1.977661652450257
  19.600000000000001   1.977661652450257
  19.800000000000001   1.977661652450257
  20.000000000000000   1.977661652450257

